BERTering RAMS: What and How Much does BERT Already Know About Event Arguments? -- A Study on the RAMS Dataset

Using the attention map based probing frame-work from (Clark et al., 2019), we observe that, on the RAMS dataset (Ebner et al., 2020), BERT's attention heads have modest but well above-chance ability to spot event arguments sans any training or domain finetuning, vary-ing from a low of 17.77% for Place to a high of 51.61% for Artifact. Next, we find that linear combinations of these heads, estimated with approx 11% of available total event argument detection supervision, can push performance well-higher for some roles - highest two being Victim (68.29% Accuracy) and Artifact(58.82% Accuracy). Furthermore, we investigate how well our methods do for cross-sentence event arguments. We propose a procedure to isolate "best heads" for cross-sentence argument detection separately of those for intra-sentence arguments. The heads thus estimated have superior cross-sentence performance compared to their jointly estimated equivalents, albeit only under the unrealistic assumption that we already know the argument is present in an-other sentence. Lastly, we seek to isolate to what extent our numbers stem from lexical frequency based associations between gold arguments and roles. We propose NONCE, a scheme to create adversarial test examples by replacing gold arguments with randomly generated "nonce" words. We find that learnt linear combinations are robust to NONCE, though individual best heads can be more sensitive.

==> sections/background.tex <==
\subsection{Problem Complexity}
Let $n$ be the number of candidates and $b$ the number of blanks. For our case, with a typical $n=7$ and $b=5$, the size of the answer space, $|A|$ is given by
\begin{align*}
    |A| &= C(n,b) \times b! \\
        &= C(7,5) \times 5! \\
        &= \frac{7(7-1)}{2} \times 120 \\
        &= 2520
\end{align*}
Thus, the \% chance of guessing all passage blanks exactly right at random is very low, precisely,  $\frac{1}{2520} \times 100 = 0.03\%$. 

What are the chances of getting answers partially correct? In particular, consider the number of answer permutations which get  atleast one blank correct, denoted by $\zeta(n,b)$. If we have the same number of candidates as blanks, this is equivalent to $b! - D_{b}$, where $D_{b}$ is the number of derangements\footnote{\url{en.wikipedia.org/wiki/Derangement}} of $b$ elements. In the presence of more candidates than blanks i.e distractors, this expression becomes more involved to derive. We defer the derivation to Appendix \S 1.2 for paucity of space. With $n=7$ and $b=5$, $\zeta(n,b)=1306$, or $51.8\%$. In other words, there is a $48.17$\% probability of being entirely wrong with a randomly chosen set of answers to each blank in the passage. \xiang{I will add derivation to the appendix.}

==> sections/intro_0117.tex <==
\vg{Overall Comment: Normalize the usage of terms: attention map/attention head}

%to be composed downstream by a task-specific model

Going one step beyond per-word-type pretrained vectors \cite{pennington2014glove} , or direct per-sentence, "squished" vectors \cite{conneau2017supervised},  contextual embeddings produce in-context representations for each token - the representation in-effect being a large, pretrained encoder. The typical procedure to use these models for a downstream task is to add one or more layers [also called ``\textit{heads}"] atop each token representation, or for a designated token per-sentence, depending on the nature of the task.

The head and the representation are then together trained, or ``\textit{finetuned}" using the task-loss, albeit with a slower training rate than would be used for training an architecture 
from scratch. ElMo \cite{peters2018deep} was one of the earliest  . Contextual representations with a transformer based model, masked language modelling objectives and large generic pre-training corpora, starting with Bert \cite{devlin2018bert} and RoBerta \cite{liu2019roberta} - proved vastly effective on most typical NLP tasks.

The good performance of contextual representations with minimal finetuning and only shallow projections made it important to understand what and how much these models \emph{already knew} about different aspects of syntax and semantics. This was important for the following reasons
\begin{enumerate}
    \item Explaining their strong performance, as also explaining in what way they were featurizing raw sentences for a given task.
    \item Finding lacunae to be addressed by future contextual representation approaches.
    \item Deciding how much task-specific training data for finetuning was necessary.
    \item This could also guide decisions about hyperparameters (learning rate) or guide inductive bias for the task-specific head architecture.
\end{enumerate}
This whole activity has come to be referred to as \emph{probing}. 

\cite{linzen2016assessing}, one of the early works on probing, evaluated whether language models could predict the correct noun form agreeing with the verb form given in the  left context. \cite{marvin2018targeted} generalized this approach beyond right, single-word gaps with a larger suite of ``minimal pairs". They also control for lexical confounding and expand the probing to new aspects such as reflexive anaphora and NPIs. \cite{gulordava2018colorless} evaluate subject-verb agreement but only through ``nonce" sentences to control for both lexical confounding and memorization.
\cite{lakretz2019emergence} isolate units of LSTM language models whose activations closely track verb-noun number agreement, particularly for hard, long-distance cases.  

\cite{hewitt2019structural} find that BERT token representations are linearly projectable into a space where they embed hierarchical constituency structure.

\cite{hewitt2019designing} raised a note of caution about classifier based probes, pointing out that probes themselves could be rich enough to learn certain phenomena even with a random representation, and propose the use of ``control tasks" as a baseline to normalize classifier probe performance. \cite{van2019quantity} probe increasing LM network sizes for their synctactic abilities and find training size to be not useful beyond a threshold.

Recently, \cite{sorodoc2020probing} probed transformer based language models for coreference. However, they restrict themselves to entity coreference. Furthermore, they restrict themselves to true (i.e left-to-right) LMs, excluding MLMs like \textsc{BERT}

Other aspects studied include filler-gap dependencies \cite{wilcox2018rnn}, function word comprehension \cite{kim2019probing}, sentence-level properties \cite{adi2016fine} and negative polarity items \cite{warstadt2019investigating}.

In this work, we venture to probe what and how much a pretrained BERT representation already knows about events and their arguments. Understanding how well event arguments are represented can be a first foray into understanding other aspects about events. Extraction of event arguments is often a prerequisite for more complex event tasks such as event coreference \cite{lu2018event}, detecting event-event temporal \cite{vashishtha2019fine}  and causal relations \cite{dunietz2017because}, and sub-event structure \cite{araki2014detecting}. Tuples of event-type and arguments are one way of inducing script like-structures \cite{chambers2008unsupervised}.


\begin{figure*}[!ht]
    \centering
    \includegraphics[width=1.9\columnwidth]{Plots/Place/attention_map_evt004arg04place_example47_Good_Cropped.png}
    \caption{In this example, the head chosen by \textsc{BestHead} for the \textsc{Place} role, correctly out the argument ``\textit{Syria}" for the trigger ``\textit{capitulation}".
    Attention probabilities are represented as blue lines from trigger position to other tokens, with width indicating magnitude. It manages to evade distractor pronouns (\textit{there}) and other geographical entity names (\textit{Russia} and \textit{United States}). The text above flows in right to left direction. The  full text goes something like: ``\textit{The chances of intentional conflict are real as is the possibility of an unintended clash escalating . At the same time, Syria is not essential to the national security of Russia or the United States. It is not without importance but a defeat or \textbf{capitulation} there will not change the balance of power between them at all \ldots}" }
    \label{fig:place39}
    % \vspace{-1ex}
\end{figure*}


In summary, our work makes the following contributions:
\begin{itemize}
    \item We show that always exists a BERT attention head with above-chance ability to detect arguments, for a given event role. We also show that this ability is even stronger through learnt linear combinations of heads.
    \item We notice a relative weakness at detecting cross sentence arguments. Motivated by this, we devise a procedure to isolate only the cross-sentence argument detection ability of heads w.r.t a role. Our procedure considerably improves cross-sentence performance for some roles such as \textsc{Instrument} and \textsc{Place}.
    \item Lastly, we devise a nonce-word based method to isolate how much of the zero-shot argument detection ability originates from commonsense and frequency statistics. We find that for $x$ types of roles it does, and for $y$ types of roles it does not.
\end{itemize}
